Polygonal Cone Control Barrier Functions (PolyC2BF) for safe navigation in cluttered environments

In fields such as mining, search and rescue, and archaeological exploration, ensuring real-time, collision-free navigation of robots in confined, cluttered environments is imperative. Despite the value of established path planning algorithms, they often face challenges in convergence rates and handling dynamic infeasibilities. Alternative techniques like collision cones struggle to accurately represent complex obstacle geometries. This paper introduces a novel category of control barrier functions, known as Polygonal Cone Control Barrier Function (PolyC2BF), which addresses overestimation and computational complexity issues. The proposed PolyC2BF, formulated as a Quadratic Programming (QP) problem, proves effective in facilitating collision-free movement of multiple robots in complex environments. The efficacy of this approach is further demonstrated through PyBullet simulations on quadruped (unicycle model), and crazyflie 2.1 (quadrotor model) in cluttered environments.

==> literature_review.tex <==


% For effective collision avoidance and ensuring safety, algorithm used should be generic i.e. should work in both static \& dynamic environment; and robust i.e. should act rapidly according to the motion of obstacle. Some local planners like A* and Dijkstra's algorithm have proposed to tackle the problem, but they show good outcomes only in static environments. On the other hand, algorithms like D*, RA*, and RRTs work well in a dynamic environment but are computationally expensive, which might not effectively avoid the collision in the scenarios with a significantly high velocity of the ego vehicle or the obstacle. Moreover, all the algorithms mentioned above do not guarantee an optimum solution and thus safety \cite{vehicles3030027}. 

% The QP-based methodology of CBF handles multiple obstacles that appear dynamically, and the QP regulates the control inputs in a minimally invasive fashion, paving the way for obstacle avoidance via circumnavigating or braking. 
%\Stanley controller \cite{4282788}

% Collision cone was formally introduced in \cite{Fiorini1993} \cite{doi:10.1177/027836499801700706} , 
The idea of collision cones was first introduced in \cite{Fiorini1993, doi:10.1177/027836499801700706, 709600} as a means to geometrically represent the possible set of velocity vectors of the vehicle that lead to collision. %\cite{709600} explores the use of collision cones for moving obstacles, discuss the calculation of the point of collision, and generalized construction of the collision cones. 
The approach was extended for irregular shaped robots and obstacles with unknown trajectories both in 2D \cite{709600} and 3D space \cite{Chakravarthy2012}. 
This was commonly used for aerospace applications like missile guidance \cite{doi:10.2514/1.G005879} and conflict detection and resolution in aircrafts \cite{doi:10.2514/6.2004-4879}. This was further extended to Model Predictive Control by formulating the cones as constraints \cite{babu2018model}.
%where a cone geometrically represents the collision region in the velocity space. %An avoidance maneuver is then planned simply by selecting a relative velocity vector that points outside of the obstacle collision cone. 
In our work, we combine the collision cone approach with CBFs to develop a novel obstacle avoiding algorithm for UGVs. With the benefits of both CBFs and Collision cone model, our C3BF algorithm is computationally efficient, works well in both static \& dynamics environments, and guarantees safety. We will demonstrate this both in simulation and experiments. % (Section III \& IV). % for the acceleration controlled UGVs (unicycle \& bicycle models).
